PatchBackdoor: Backdoor Attack against Deep Neural Networks without Model Modification

Backdoor attack is a major threat to deep learning systems in safety-critical scenarios, which aims to trigger misbehavior of neural network models under attacker-controlled conditions. However, most backdoor attacks have to modify the neural network models through training with poisoned data and/or direct model editing, which leads to a common but false belief that backdoor attack can be easily avoided by properly protecting the model. In this paper, we show that backdoor attacks can be achieved without any model modification. Instead of injecting backdoor logic into the training data or the model, we propose to place a carefully-designed patch (namely backdoor patch) in front of the camera, which is fed into the model together with the input images. The patch can be trained to behave normally at most of the time, while producing wrong prediction when the input image contains an attacker-controlled trigger object. Our main techniques include an effective training method to generate the backdoor patch and a digital-physical transformation modeling method to enhance the feasibility of the patch in real deployments. Extensive experiments show that PatchBackdoor can be applied to common deep learning models (VGG, MobileNet, ResNet) with an attack success rate of 93% to 99% on classification tasks. Moreover, we implement PatchBackdoor in real-world scenarios and show that the attack is still threatening.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tex/defense/base.tex <==
\section{Defenses}
\subsection{Activation Cluster}

In this experiment, we used CIFAR10(32*32) to conduct attack. The patch is top left bar with width 7. The trigger is a grey block with width 3. Locating at the top left corner of the

Activation cluster\cite{AC}(AC) is a backdoor defense method targeting detection and removing the data poisoning attack. The key idea is although the poisoned sample has the same classification as normal samples, the path of the activations was different. In other words, the features that cause the poisoned sample to be classified as the target class differ from the features that cause the clean sample to be classified as the same class(The target class must also have its corresponding clean data.). The activation cluster detects the backdoor attack by analyzing the activation before the last layer. Their experiment has shown the activation of the last hidden layer could be separated if clean samples are mixed with poisoned samples. Then they came up with several ways to determine whether the cluster is abnormal. If the dataset is clean, there should be only one cluster, which will be inappropriate to separate. However, if the dataset is poisoned, then the separation of the cluster is clear.

The first evaluation metric requires retraining the model. However, that only corresponds to those attacks that need to modify the model. It is unreasonable to retrain a model if no one has changed it after deployment. The training is also time-taken since it requires training a new model instead of fine-tuning.

% \begin{table*}
% 	\caption{Defense result for Activation Clustering}
% 	\vspace{-0.3cm}
% 	\centering
% 	\resizebox{.47\textwidth}{!}
%     {
% 	\begin{tabular}{crr}
% 		\toprule
% 		%\multicolumn{2}{c}{Part}                   \\
% 		\cmidrule(r){1-2}
% 		class    &  \% in Cluster 0   & \% in Cluster 1 & Silhouette Score \\
% 		\midrule
%         class0	&49\%	&51\%	&0.0014\\
%         class1	&50\%	&50\%	&0.0007\\
%         class2	&49\%	&51\%	&0.0002\\
%         class3	&49\%	&51\%	&0.0002\\
%         class4	&48\%	&52\%	&0.0046\\
%         class5	&48\%	&52\%	&0.0026\\
%         class6	&48\%	&52\%	&0.0032\\
%         class7	&49\%	&51\%	&0.0014\\
%         class8	&49\%	&51\%	&0.0\\
%         class9	&50\%	&50\%	&0.0004\\
% 		\bottomrule
% 	\end{tabular}
%     }
% 	\label{tab:ac}
% \end{table*}   
\oracle{I need to keep mention AC paper several times, how should I do that?}
The second way and the third way of detecting if the cluster separation is reasonable is cluster size ratio and Sihouette score. The suggested threshold for Sihouette score is between 0.10 and 0.15, all clean dataset in the AC paper has a lower Sihouette score . Based on ~\ref{tab:ac}, we can see our Sihouette score is far below the suggested upperbound. For relative size, the most uneven distribute of all dataset in AC paper is 30\% and 70\%. Our separation is much more even than that. Based on AC paper's idea, our dataset is clean.


==> tex/evaluation/pruning.tex <==
\begin{figure}
    \centering
    \includegraphics[width=8cm]{pics/PruningBetter.png}
	\vspace{-0.2cm}
    \caption{The attack effectiveness of \sys on models with different sizes and pruning ratios.}
    \label{fig:pruning}
    % \vspace{-0.2cm}
\end{figure}

It is a common belief that the robustness of a model is related to the over-parameterization \cite{robustOverParameterization}.
So we examine whether the attack effectiveness of our method may be affected by different levels of over-parameterization. Specifically, we test our attack on models with different sizes and varying pruning ratios. The dataset used in this experiment is Imagenette, and the models include VGG11, VGG16, ResNet50, and ResNet101. The patch width is 40 pixels and the trigger width is 30 pixels. The pruning algorithm is L1 norm-based global pruning \cite{L1Pruning}. \oracle{For each combination of model and pruning ratio, we train the backdoor patches with the same hyperparameters for the same number of epochs after pruning. For a detailed analysis of the training patch before pruning, please refer to Section \ref{sec:robust} }

As demonstrated in Figure \ref{fig:pruning}, the levels of over-parameterization do not significantly influence the success of \sys attacks. For the diverse models and pruning ratios, \sys achieved a consistently high attack success rate with negligible reduction in clean accuracy. This indicates that most models possess a substantial degree of redundant parameters; despite diminishing the number of parameters, the attack can still be successfully executed.
Meanwhile, the attack success rates on the original models (pruning ratio=0\%) are slightly better, which implies that the more redundant parameters can be more easily utilized to inject the backdoor logic, although the difference is rather small.



==> tex/problemStatement.tex <==
\begin{table*}[]
        \centering
        \caption{The difference between our attack and common existing attacks. \yuanchun{what is controllable activation?}}
        \begin{tabular}{c c c c c}
                \toprule
                Method & No Model Modification & Aribitary Trigger & Physical-world Feasibility & Controllable Activation \\ \midrule
                Backdoor Attack & No & Yes & No & Yes\\ 
                Adversarial Patch & Yes &No&Yes&No\\ 
                Adversarial Purturbation & Yes & No & No & Yes\\ \hline
                \sys &Yes &Yes &Yes &Yes\\ \bottomrule
                
        \end{tabular}
        % }
        \label{table:compare}
        % \vspace{-10pt}
        \end{table*} 

\section{Problem Formulation}
\subsection{Threat Model}
% \yuanchun{Normally `Threat Model' comes before `Problem Statement'}
% \oracle{Done}

Suppose there is a deep learning-based vision model deployed in the physical world. The model takes the image captured by a camera as the input, and the camera view contains a constant foreground or background (\eg a wall or a car hood near the camera).
The attacker can inject a backdoor logic (\ie letting the model behavior as usual in most of the time, while producing wrong predictions if the input image satisfies an attacker-defined condition) by attaching a patch onto the constant foreground/background in the camera view.
We assume the attacker has read access to the victim model, so that it can use the model weights to do backward propagation. However, it is impossible for the attacker to modify the model weights.
Moreover, unlike most backdoor attack approaches, we assume that the attacker have no read or write access to the original training data.
%  However, compared to other white box backdoor attacks, we do not need to modify the model's weight, which makes the attack much more applicable.
% We also assume there were human defenders with models. If the model has misprediction when they see suspicious pictures, they will think it is an adversarial patch. If the model performs normally, they will think it is some art, which is a reasonable assumption nowadays. 

\subsection{Problem Statement}\label{3}
% \oracle{I don`t know if this is ok...}
Recall the formula in Equation~\ref{equation:backdoor}, the objective of our attack is almost the same as the backdoor attack. However, instead of modifying the victim model $f$ to a new model $f'$, we keep the model $f$ as is. Our patch is denoted as $p$, and $x \oplus p$ means to attach the patch $p$ to the image $x$. The attack trigger condition is denoted as $c$, and $x \oplus c$ represents the input image that satisfies the trigger condition, \eg a trigger object is present in the image, the image is in certain lighting condition, etc.
% However, the normal state could be special too. For example, the green light means to disable the attack, while the red light means to turn on the attack. In that case, green light is considered as default with no additional notation while red light is the attack condition which is denoted as $\oplus c$. 
Therefore, our attack aims to maximize following two probabilities:
\begin{equation}
P(f(x\oplus p \oplus c)=\hat{y}),\ \ P(f(x\oplus p)=y_{target})
\label{equation:cap}
\end{equation}


  




 
